Simulation-based Analysis of Multipath Delay Distributions in Urban Canyons

Global navigation satellite systems provide accurate positioning nearly worldwide. However, in the urban canyons of dense cities, buildings block and reflect the signals, causing multipath errors. To mitigate multipath errors, knowledge of the distribution of the reflection delays is important. Measurements of this distribution have been done in several dense cities, but it is unknown how the delay distribution depends on the depth of the urban canyon. To fill this gap, we simulated reflection scenarios in 12 different environments: from suburban to deep urban canyon. Subsequently, we analyzed the resulting delay distributions. This paper presents these distributions, and a method to estimate them using the number of received satellites. According to our simulation, the multipath delays follow gamma distributions, whose shape parameters decrease when the urban canyon depth increases. A quadratic model can estimate the shape parameter using the number of received satellites. Consequently, depending on the number of received satellites, the distribution of the reflection delays can be estimated. This information can be combined with prior knowledge from other methods for improved multipath delay estimation. In the future, for more realistic results, the effects on signals that are reflected multiple times and environments other than urban canyons should be simulated.

==> ENC.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%  Definitions for the first page,                
%%%  the headlines and the footing       
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\setlength{\parindent}{0mm}
\setlength{\parskip}{1em}
\footskip0mm
\topmargin-0.4mm
\headheight0mm
\headsep0mm
\evensidemargin-0.4mm
\oddsidemargin-0.4mm
\textwidth160mm
\textheight231mm
\renewcommand{\baselinestretch}{1.05}
\frenchspacing
\sloppy


\pagestyle{empty}


\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.5}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.6}


%  Spacing shorthands
\newcommand {\hsp}   {\hspace*}
\newcommand {\vsp}   {\vspace*}
\newcommand {\fns}   {\footnotesize}
\newcommand {\ens}   {\enspace}
\newcommand {\bu}    {\bullet\hsp{1mm}}
\newcommand {\hx}    {{\small\raisebox{.8pt}{x}}}


   
\def\title#1{\vsp{-16mm}\begin{center}\Large\bf{#1}\end{center}\vsp{0mm}}
\def\author#1{{\begin{center}\textbf{#1}\end{center}\vspace{-1mm}}}
\def\address#1{\vsp{-3mm}\begin{center}\baselineskip12pt\normalsize{#1}\end{center}\vsp{-1mm}}
\def\keywords#1{\vspace{7mm}{\bf Key words:\hsp{3mm}\rm{#1}\vspace{0mm}}}
\def\abstract#1{{\vspace{-5mm}
    \begin{center}
      \begin{minipage}{0.85\textwidth}
        \noindent\bf \textit{Abstract:}
        \small\rm\emph{#1}
				\vsp{-0.5em}
      \end{minipage}
    \end{center}
}}

\def\authorsheadline=#1{\global\def\@authorsheadline{#1}}
\global\def\@authorsheadline{}



\def\TeX{T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}

\def\LaTeXG{{\rm L\kern-.36em\raise.3ex\hbox{\sc a}\kern-.15emT\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\LaTeXK{{\it L\kern-.24em\raise.4ex\hbox{\scriptsize \it A}\kern-.20emT\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}


\jot 4pt
\setcounter{secnumdepth}{3}

